Formal Verification of the Empty Hexagon Number

A recent breakthrough in computer-assisted mathematics showed that every set of $30$ points in the plane in general position (i.e., without three on a common line) contains an empty convex hexagon, thus closing a line of research dating back to the 1930s. Through a combination of geometric insights and automated reasoning techniques, Heule and Scheucher constructed a CNF formula $\phi_n$, with $O(n^4)$ clauses, whose unsatisfiability implies that no set of $n$ points in general position can avoid an empty convex hexagon. An unsatisfiability proof for n = 30 was then found with a SAT solver using 17300 CPU hours of parallel computation, thus implying that the empty hexagon number h(6) is equal to 30. In this paper, we formalize and verify this result in the Lean theorem prover. Our formalization covers discrete computational geometry ideas and SAT encoding techniques that have been successfully applied to similar Erd\H{o}s-Szekeres-type problems. In particular, our framework provides tools to connect standard mathematical objects to propositional assignments, which represents a key step towards the formal verification of other SAT-based mathematical results. Overall, we hope that this work sets a new standard for verification when extensive computation is used for discrete geometry problems, and that it increases the trust the mathematical community has in computer-assisted proofs in this area.

==> empty_triangle.tex <==
Let us consider a much simpler theorem, which we call the \emph{empty triangle theorem}. Its proof will be helpful to motivate the different aspects of our formalization of the empty hexagon theorem.

\begin{theorem}[Empty Triangle Theorem]
  \label{thm:empty-triangle}
  Given a set $S$ of $n \geq 3$ points in general position, there exists $3$ points $a, b, c \in S$ such that no point $d \in S$ lies inside the triangle $abc$.
\end{theorem}

\begin{proof}[(Human Proof)]
    Let $a, b, x$ be any three points of $S$.
    Define the relation $p \prec q$ to mean that the triangle $abp$ is contained inside the triangle $abq$. Note that $\prec$ is a finite partial order, and thus there must exist at least one minimal element for $\prec$.
    Let $c$ be a minimal element of $\prec$, and now note that $abc$ cannot contain any other point $d \in  S$, as otherwise we would have $d \prec c$, contradicting the minimality of $c$. An illustration of this proof is presented in~\Cref{fig:empty-triangle}.
\end{proof}

\begin{figure}
\centering
\begin{tikzpicture}
\node[draw, circle, black, fill=black, inner sep=0pt, minimum size=5pt] (h) at (0,0) {};
\node[draw, circle, black, fill=black, inner sep=0pt, minimum size=5pt] (c) at (2,3) {};
\node[] at (2, 2.75) {$c$};
\node[draw, circle, black, fill=black, inner sep=0pt, minimum size=5pt] (p) at (1.2,4.75) {};
\node[draw, circle, black, fill=black, inner sep=0pt, minimum size=5pt] (d) at (4,1) {};
\node[draw, circle, black, fill=black, inner sep=0pt, minimum size=5pt] (e) at (5,6) {};
\node[draw, circle, black, fill=black, inner sep=0pt, minimum size=5pt] (f) at (2,7) {};
\node[draw, circle, black, fill=black, inner sep=0pt, minimum size=5pt] (g) at (4,5) {};
\node[draw, circle, black, fill=black, inner sep=0pt, minimum size=5pt] (a) at (-1,2) {};
\node[] at (-1.2, 1.75) {$a$};
\node[draw, circle, black, fill=black, inner sep=0pt, minimum size=5pt] (i) at (-2,3) {};
\node[draw, circle, black, fill=black, inner sep=0pt, minimum size=5pt] (j) at (-0.5, 3.5) {};
% \node[draw, circle, black, fill=black, inner sep=0pt, minimum size=5pt] (k) at (2.5,-1) {};
\node[draw, circle, black, fill=black, inner sep=0pt, minimum size=5pt] (l) at (3,6) {};
\node[draw, circle, black, fill=black, inner sep=0pt, minimum size=5pt] (m) at (-4,2) {};
% \node[draw, circle, black, fill=black, inner sep=0pt, minimum size=5pt] (n) at (-2, -2) {};
\node[draw, circle, black, fill=black, inner sep=0pt, minimum size=5pt] (o) at (2, 0) {};

\node[draw, circle, black, fill=black, inner sep=0pt, minimum size=5pt] (b) at (5,1) {};
\node[] at (5.2, 0.75) {$b$};

\node[draw, circle, black, fill=black, inner sep=0pt, minimum size=5pt] (q) at (3.2, 3.75) {};

\draw[ultra thick, dashed, blue] (a) -- (b);
\draw[fill=green, opacity=0.5] (a.center) -- (b.center) -- (c.center) -- cycle;
\draw[dashed] (a.center) -- (b.center) -- (l.center) -- cycle;
\draw[dashed] (a.center) -- (b.center) -- (g.center) -- cycle;
\draw[dashed] (a.center) -- (b.center) -- (e.center) -- cycle;
\draw[dashed] (a.center) -- (b.center) -- (q.center) -- cycle;
\draw[dashed] (a.center) -- (b.center) -- (f.center) -- cycle;
\draw[dashed] (a.center) -- (b.center) -- (p.center) -- cycle;

\end{tikzpicture}
\caption{An illustration of the proof for~\Cref{thm:empty-triangle}.}
\label{fig:empty-triangle}
\end{figure}

Instead of formalizing the above proof, we will formalize a SAT-based proof, with the goal of approaching the formalization of the empty hexagon theorem.
Naturally, to use a  SAT-solver we need to parameterize~\Cref{thm:empty-triangle} by $n = |S|$, the number of points, and generate a different proof for each value of $n \geq 3$. For example, consider the following theorem.

\begin{lstlisting}
  theorem EmptyTriangle10Theorem (pts : Finset Point)
    (gp : PointFinsetInGenPos pts)
    (h : pts.card = 10) :
    ∃ (p q r : Point), {p, q, r} ⊆ pts ∧ EmptyTriangleIn p q r pts
\end{lstlisting}

To complete the statement of the theorem, we must define~\texttt{EmptyTriangleIn}, and before that what it means for a point to be \emph{inside} a triangle.

\begin{lstlisting}
  def pt_in_triangle (a : Point) (p q r : Point) : Prop :=
    ∃ p' q' r', ({p', q', r'} : Set Point) = {p, q, r} ∧
      Sorted₃ p' q' r' ∧
      Sorted₃ p' a r' ∧
      a ≠ q' ∧ -- this isn't needed if p,q,r are in GP
      σ p' q' r' = σ p' a r' ∧
      σ p' a q' = σ p' r' q' ∧
      σ q' a r' = σ q' p' r'

  /-- S is an empty triangle relative to pts -/
  structure EmptyTriangleIn (p q r : Point) (pts : Finset Point) : Prop :=
    gp : InGenPos₃ p q r
    empty: ∀ a ∈ pts, ¬(pt_in_triangle a p q r)
\end{lstlisting}




==> leansat.tex <==
This section describes the bridge between mathematical objects and the propositional variables representing them in the context of a CNF formula.
Consider the following theorem:

\begin{lstlisting}
theorem EmptyTriangle10TheoremLists
    (pts : List Point) (gp : PtListInGP pts) (h : pts.length = 10) :
    HasEmptyTriangle pts.toFinset
\end{lstlisting}

% We wish to prove that no list of $10$ points in general position can avoid an empty triangle.
% Consider the propositional formula $\varphi$ over variables $\orvar_{p, q, r}$, with $1 \leq p  < q < r \leq 10$.
% \begin{enumerate}
%     % \item $\left(\neg \orvar_{p, q, r} \lor \neg \orvar_{p, r, t} \lor \orvar_{p, q, t}\right) \land \left(\orvar_{p, q, r} \lor \orvar_{p, r, t} \lor  \neg \orvar_{p, q, t}\right)$
%     % &\left(\neg \orvar_{p, q, r} \lor \neg \orvar_{q, r, t} \lor  \orvar_{p, r, t}\right) \land \left(\orvar_{p, q, r} \lor \orvar_{q, r, t} \lor  \neg \orvar_{p, r, t}\right).
% \end{enumerate}





% Describe how we go from abstract formula over boolean variables
% to a CNF using encoding programs.
% CNF is usually large, and SAT solvers take the CNF in a format called DIMACS which is not human inspectable.
% Thus usually generated by encoding program rather than constructed manually.
% This DIMACS is fed to a SAT solver, which produces an UNSAT certificate
% (usually in a format known as DRAT or LRAT).

% Given this pipeline, we have two distinct concerns for correctness:
% \begin{itemize}
%     \item[(1)] \textbf{Is the CNF formula correct?}
%     We want to formally verify that our ``encoder'' program
%     generates DIMACS output which
%     correctly represent the abstract formula we wish to show UNSAT.
%     \item[(2)] \textbf{Is the SAT solver output correct?}
%     The UNSAT certificate must be checked for correctness
%     against the DIMACS formula.
% \end{itemize}

% Prior work on (2) has produced highly trustworthy proof checkers
% for SAT solver output (cake lpr citation, GRAT citation maybe?).
% We rely on \texttt{cake\_lpr} for this step of the proof,
% and trust that the DIMACS formula given to \texttt{cake\_lpr}
% is unsatisfiable if this program terminates without error.

% In contrast, we found very little prior work on (1).
% Codel (cite Codel, any other papers Cayden found about this).

% We built on (bryant citation, codel citation)
% to develop tools for writing correct-by-construction encoding programs
% against an abstract model of propositional formulas.
% This infrastructure is a component of the fledgling \leansat{} library,
% which is largely outside the scope of this paper.
% Nonetheless this library enabled us to re-implement
% Heule et al's encoding exactly as presented (TODO: is this true?).

% Here we give a brief overview of how this section of the formalization proceeds.

% \subsection{Variables}

% The \leansat{} library allows formulas to be written over arbitrary variable sets.
% As an example, for the Empty Triangle Theorem (see section 5) we use the following variables:
% \begin{lstlisting}
% inductive Var (n : Nat)
%   | sigma  (a b c : Fin n)
%   | inside (x a b c : Fin n)
%   | hole   (a b c : Fin n)
% \end{lstlisting}
% TODO explain how the library handles converting these variables to \(\mathbb{N}\)
% for the purposes of DIMACS.

% \subsection{Abstract Propositional Formula}

% Given that the encoding presented in Heule et al has many sets of clauses,
% we divide the abstract formula into a few sub-formulas.
% Here is the formula which defines the "is hole" variables:
% \begin{lstlisting}
% /--
%   Triangle abc is a hole iff all x are not inside triangle abc.
% -/
% def holeDefs (n : Nat) : PropAssignment (Var n) → Prop := fun τ =>
%   ∀ {a b c}, τ (Var.hole a b c) ↔
%     (∀ x, a < x → x < c → x ≠ b →
%       !τ (Var.inside x a b c))
% \end{lstlisting}
% The Lean statement here is clean and simple,
% and nicely corresponds to the paper presentation.
% We define the entire formula in around 100 lines of Lean.
% TODO(JG): get exact numbers

% \subsection{Encoding Program}

% Now that we have defined an abstract formula over our variables,
% we need to write a program which encodes this formula to DIMACS.
% Again we divide the program into sub-programs,
% corresponding exactly to how we divided up the formula.
% Here is the signature of the encoder for the formula from the previous section:
% \begin{lstlisting}
% def holeDefClauses (n : Nat) : VEncCNF (Var n) Unit (holeDefs n) :=
%   ...
% \end{lstlisting}
% The \texttt{VEncCNF} type is essentially a state monad,
% where the state is the DIMACS output.
% However, it is constrained to those programs which
% verifiably encode the predicate \texttt{holeDefs n}.

% In particular, if we run \texttt{holeDefClauses n},
% we get DIMACS output which is satisfiable iff \texttt{holeDefs n} is satisfiable,
% no matter what the particulars are in \texttt{holeDefClauses}.
% This is expressed in the following theorem from \leansat{}:
% \begin{lstlisting}
% theorem toICnf_equisatisfiable [FinEnum ν] (v : VEncCNF L α P) :
%   (∃ τ : PropAssignment IVar, τ |= v.val.toICnf.toPropFun) ↔
%     (∃ τ : PropAssignment ν, P τ)
% \end{lstlisting}
% TODO(JG): cleanup in leansat

% The encoding program, and its verification,
% takes a few hundred lines of Lean.
% TODO(JG) update when done rewriting

% \subsection{Verifying UNSAT Proof}

% We have generated a DIMACS-format formula which is satisfiable iff
% our abstract encoding is satisfiable.
% Ideally, at this point we would emit the formula,
% run a SAT solver,
% get a proof of unsatisfiability,
% and then check this proof \textit{in the trusted Lean kernel}.
% This approach would establish the formula unsatisfiable
% with the same level of trust as all mathematics verified in Lean.

% Unfortunately, such an approach is not feasible due to performance constraints.
% The Lean kernel is simple and trustworthy,
% but evaluates programs quite slowly,
% orders of magnitude slower than executing compiled Lean programs.
% The \(h(6) = 30\) result generated on the order of 100 TB of DRAT proof,
% which is far, far beyond the range at which the kernel could feasibly check.

% TODO(JG): explain our new trust story for this last leg of the journey.

% \begin{lstlisting}
% axiom cnfUnsat : ¬∃ τ, τ |= (theEncoding 30).toICNF
% \end{lstlisting}
% TODO(JG): make this statement reality


==> lstlean.tex <==
% Listing style definition for the Lean Theorem Prover.
% Defined by Jeremy Avigad, 2015, by modifying Assia Mahboubi's SSR style.
% Unicode replacements taken from Olivier Verdier's unixode.sty

\lstdefinelanguage{lean} {

% Anything between $ becomes LaTeX math mode
mathescape=false,
% Comments may or not include Latex commands
texcl=false,

% keywords, list taken from lean-syntax.el
morekeywords=[1]{
import, prelude, protected, private, noncomputable, definition, meta, renaming,
hiding, parameter, parameters, begin, constant, constants,
lemma, variable, variables, theory,
print, theorem, example,
open, as, export, override, axiom, axioms, inductive, with,
structure, record, universe, universes,
alias, help, precedence, reserve, declare_trace, add_key_equivalence,
match, infix, infixl, infixr, notation, postfix, prefix, instance,
eval, reduce, check, end, this,
using, using_well_founded, namespace, section,
attribute, local, set_option, extends, include, omit, class,
raw, replacing,
calc, have, show, suffices, by, in, at, let, forall, Pi, fun,
exists, if, dif, then, else, assume, obtain, from, register_simp_ext, unless, break, continue,
mutual, do, def, run_cmd, const,
partial, mut, where, macro, syntax, deriving,
return, try, catch, for, macro_rules, declare_syntax_cat, abbrev},

% Sorts
morekeywords=[2]{Sort, Type, Prop},

% tactics, list taken from lean-syntax.el
morekeywords=[3]{
assumption,
apply, intro, intros, allGoals,
generalize, clear, revert, done, exact,
refine, repeat, cases, rewrite, rw,
simp, simp_all, contradiction,
constructor, injection,
induction,
},

% modifiers, taken from lean-syntax.el
% note: 'otherkeywords' is needed because these use a different symbol.
% this command doesn't allow us to specify a number -- they are put with [1]
% otherkeywords={
% [persistent], [notation], [visible], [instance], [trans_instance],
% [class], [parsing-only], [coercion], [unfold_full], [constructor],
% [reducible], [irreducible], [semireducible], [quasireducible], [wf],
% [whnf], [multiple_instances], [none], [decl], [declaration],
% [relation], [symm], [subst], [refl], [trans], [simp], [congr], [unify],
% [backward], [forward], [no_pattern], [begin_end], [tactic], [abbreviation],
% [reducible], [unfold], [alias], [eqv], [intro], [intro!], [elim], [grinder],
% [localrefinfo], [recursor]
% },

% Various symbols
literate=
{α}{{\ensuremath{\mathrm{\alpha}}}}1
{β}{{\ensuremath{\mathrm{\beta}}}}1
{γ}{{\ensuremath{\mathrm{\gamma}}}}1
{δ}{{\ensuremath{\mathrm{\delta}}}}1
{ε}{{\ensuremath{\mathrm{\varepsilon}}}}1
{ζ}{{\ensuremath{\mathrm{\zeta}}}}1
{η}{{\ensuremath{\mathrm{\eta}}}}1
{θ}{{\ensuremath{\mathrm{\theta}}}}1
{ι}{{\ensuremath{\mathrm{\iota}}}}1
{κ}{{\ensuremath{\mathrm{\kappa}}}}1
{μ}{{\ensuremath{\mathrm{\mu}}}}1
{ν}{{\ensuremath{\mathrm{\nu}}}}1
{ξ}{{\ensuremath{\mathrm{\xi}}}}1
{π}{{\ensuremath{\mathrm{\mathnormal{\pi}}}}}1
{ρ}{{\ensuremath{\mathrm{\rho}}}}1
{σ}{{\ensuremath{\mathrm{\sigma}}}}1
{τ}{{\ensuremath{\mathrm{\tau}}}}1
{φ}{{\ensuremath{\mathrm{\varphi}}}}1
{χ}{{\ensuremath{\mathrm{\chi}}}}1
{ψ}{{\ensuremath{\mathrm{\psi}}}}1
{ω}{{\ensuremath{\mathrm{\omega}}}}1

{Γ}{{\ensuremath{\mathrm{\Gamma}}}}1
{Δ}{{\ensuremath{\mathrm{\Delta}}}}1
{Θ}{{\ensuremath{\mathrm{\Theta}}}}1
{Λ}{{\ensuremath{\mathrm{\Lambda}}}}1
{Σ}{{\ensuremath{\mathrm{\Sigma}}}}1
{Φ}{{\ensuremath{\mathrm{\Phi}}}}1
{Ξ}{{\ensuremath{\mathrm{\Xi}}}}1
{Ψ}{{\ensuremath{\mathrm{\Psi}}}}1
{Ω}{{\ensuremath{\mathrm{\Omega}}}}1

{ℵ}{{\ensuremath{\aleph}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1
{≠}{{\ensuremath{\neq}}}1
{≈}{{\ensuremath{\approx}}}1
{≡}{{\ensuremath{\equiv}}}1
{≃}{{\ensuremath{\simeq}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1

{∂}{{\ensuremath{\partial}}}1
{∆}{{\ensuremath{\triangle}}}1 % or \laplace?

{∫}{{\ensuremath{\int}}}1
{∑}{{\ensuremath{\mathrm{\Sigma}}}}1
{Π}{{\ensuremath{\mathrm{\Pi}}}}1

{⊥}{{\ensuremath{\perp}}}1
{∞}{{\ensuremath{\infty}}}1
{∂}{{\ensuremath{\partial}}}1

{∓}{{\ensuremath{\mp}}}1
{±}{{\ensuremath{\pm}}}1
{×}{{\ensuremath{\times}}}1

{⊕}{{\ensuremath{\oplus}}}1
{⊗}{{\ensuremath{\otimes}}}1
{⊞}{{\ensuremath{\boxplus}}}1

{∇}{{\ensuremath{\nabla}}}1
{√}{{\ensuremath{\sqrt}}}1

{⬝}{{\ensuremath{\cdot}}}1
{•}{{\ensuremath{\cdot}}}1
{∘}{{\ensuremath{\circ}}}1

%{⁻}{{\ensuremath{^{\textup{\kern1pt\rule{2pt}{0.3pt}\kern-1pt}}}}}1
{⁻}{{\ensuremath{^{-}}}}1
{▸}{{\ensuremath{\blacktriangleright}}}1

{⊤}{{\ensuremath{\top}}}1
{∧}{{\ensuremath{\wedge}}}1
{∨}{{\ensuremath{\vee}}}1
{¬}{{\ensuremath{\neg}}}1
{⊢}{{\ensuremath{\vdash}}}1
{⊨}{{\ensuremath{\models}}}1

%{⟨}{{\ensuremath{\left\langle}}}1
%{⟩}{{\ensuremath{\right\rangle}}}1
{⟨}{{\ensuremath{\langle}}}1
{⟩}{{\ensuremath{\rangle}}}1

{↦}{{\ensuremath{\mapsto}}}1
{←}{{\ensuremath{\leftarrow}}}1
{<-}{{\ensuremath{\leftarrow}}}1
{→}{{\ensuremath{\rightarrow}}}1
{↔}{{\ensuremath{\leftrightarrow}}}1
{⇒}{{\ensuremath{\Rightarrow}}}1
{⟹}{{\ensuremath{\Longrightarrow}}}1
{⇐}{{\ensuremath{\Leftarrow}}}1
{⟸}{{\ensuremath{\Longleftarrow}}}1

{∩}{{\ensuremath{\cap}}}1
{∪}{{\ensuremath{\cup}}}1
{⊂}{{\ensuremath{\subseteq}}}1
{⊆}{{\ensuremath{\subseteq}}}1
{⊄}{{\ensuremath{\nsubseteq}}}1
{⊈}{{\ensuremath{\nsubseteq}}}1
{⊃}{{\ensuremath{\supseteq}}}1
{⊇}{{\ensuremath{\supseteq}}}1
{⊅}{{\ensuremath{\nsupseteq}}}1
{⊉}{{\ensuremath{\nsupseteq}}}1
{∈}{{\ensuremath{\in}}}1
{∉}{{\ensuremath{\notin}}}1
{∋}{{\ensuremath{\ni}}}1
{∌}{{\ensuremath{\notni}}}1
{∅}{{\ensuremath{\emptyset}}}1

{∖}{{\ensuremath{\setminus}}}1
{†}{{\ensuremath{\dag}}}1

{ℕ}{{\ensuremath{\mathbb{N}}}}1
{ℤ}{{\ensuremath{\mathbb{Z}}}}1
{ℝ}{{\ensuremath{\mathbb{R}}}}1
{ℚ}{{\ensuremath{\mathbb{Q}}}}1
{ℂ}{{\ensuremath{\mathbb{C}}}}1
{⌞}{{\ensuremath{\llcorner}}}1
{⌟}{{\ensuremath{\lrcorner}}}1
{⦃}{{\ensuremath{\{\!|}}}1
{⦄}{{\ensuremath{|\!\}}}}1

{‖}{{\ensuremath{\|}}}1
{₁}{{\ensuremath{_1}}}1
{₂}{{\ensuremath{_2}}}1
{₃}{{\ensuremath{_3}}}1
{₄}{{\ensuremath{_4}}}1
{₅}{{\ensuremath{_5}}}1
{₆}{{\ensuremath{_6}}}1
{₇}{{\ensuremath{_7}}}1
{₈}{{\ensuremath{_8}}}1
{₉}{{\ensuremath{_9}}}1
{₀}{{\ensuremath{_0}}}1
{ᵢ}{{\ensuremath{_i}}}1
{ⱼ}{{\ensuremath{_j}}}1
{ₐ}{{\ensuremath{_a}}}1

{¹}{{\ensuremath{^1}}}1

{ₙ}{{\ensuremath{_n}}}1
{ₘ}{{\ensuremath{_m}}}1
{ₚ}{{\ensuremath{_p}}}1
{ₓ}{{\ensuremath{_{\mathtt{x}}}}}1
{↑}{{\ensuremath{\uparrow}}}1
{↓}{{\ensuremath{\downarrow}}}1

{...}{{\ensuremath{\ldots}}}1
{·}{{\ensuremath{\cdot}}}1

{▸}{{\ensuremath{\triangleright}}}1

{Σ}{{\color{symbolcolor}\ensuremath{\Sigma}}}1
{Π}{{\color{symbolcolor}\ensuremath{\Pi}}}1
{∏}{{\color{symbolcolor}\ensuremath{\prod}}}1
{∀}{{\color{symbolcolor}\ensuremath{\forall}}}1
{∃}{{\color{symbolcolor}\ensuremath{\exists}}}1
{λ}{{\color{symbolcolor}\ensuremath{\mathrm{\lambda}}}}1
{\$}{{\color{symbolcolor}\$}}1

{=}{{\color{symbolcolor}=}}1
{:=}{{\color{symbolcolor}:=}}2
{=>}{{\color{symbolcolor}=>}}2
{<|>}{{\color{symbolcolor}<|>}}3
{<\$>}{{\color{symbolcolor}<\$>}}3
{+}{{\color{symbolcolor}+}}1
{~}{{\color{symbolcolor}\ensuremath{\sim}}}1
{*}{{\color{symbolcolor}*}}1
% https://tex.stackexchange.com/a/333147
{\ -\ }{{\color{symbolcolor}\ -\ }}1,

% Comments
%comment=[s][\itshape \color{commentcolor}]{/-}{-/},
morecomment=[s][\color{commentcolor}]{/-}{-/},
morecomment=[l][\itshape \color{commentcolor}]{--},

% Spaces are not displayed as a special character
showstringspaces=false,

% keep spaces
keepspaces=true,

% String delimiters
morestring=[b]",
morestring=[d],

% Size of tabulations
tabsize=3,

% Enables ASCII chars 128 to 255
extendedchars=false,

% Case sensitivity
sensitive=true,

% Automatic breaking of long lines
breaklines=true,
breakatwhitespace=true,

% Default style fors listingsred
basicstyle=\ttfamily\small,

% Position of captions is bottom
captionpos=b,

% Full flexible columns
columns=[l]fullflexible,


% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the beginning of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\color{keywordcolor}},

% Style for sorts
keywordstyle=[2]{\ttfamily\color{sortcolor}},

% Style for tactics keywords
keywordstyle=[3]{\ttfamily\color{tacticcolor}},

% Style for attributes
keywordstyle=[4]{\ttfamily\color{attributecolor}},

% Style for strings
stringstyle=\ttfamily,

% Style for comments
commentstyle={\ttfamily\footnotesize },

}

